Small Decision Trees for MDPs with Deductive Synthesis

Markov decision processes (MDPs) describe sequential decision-making processes; MDP policies return for every state in that process an advised action. Classical algorithms can efficiently compute policies that are optimal with respect to, e.g., reachability probabilities. However, these policies are then given in a tabular format. A longstanding challenge is to represent optimal or almost-optimal policies concisely, e.g., as decision trees. This paper makes two contributions towards this challenge: first, an SMT-based approach to encode a given (optimal) policy as a small decision tree, and second, an abstraction-refinement loop that searches for policies that are optimal within the set of policies that can be represented with a small tree. Technically, the latter combines the SMT encoding with verification approaches for families of Markov chains. The empirical evaluation demonstrates the feasibility of these approaches and shows how they can outperform the state-of-the-art on various benchmarks, yielding up to 20 times smaller trees representing (almost) optimal policies for models with up to 10k states and 19 variables.

==> tables/big-dtcontrol-table.tex <==
\begin{tabular}{l c@{\hskip 12pt}rrr@{\hskip 12pt}rrr}
\toprule
\multirow{2}{*}{model} &
\multicolumn{1}{c@{\hskip 12pt}}{model info} &
\multicolumn{3}{c@{\hskip 12pt}}{\dtpaynt} &
\multicolumn{3}{c}{\dtcontrol}\\
\cmidrule(lr{1.75em}){2-2}\cmidrule(lr{1.75em}){3-5}\cmidrule(lr){6-8}
& choices & time & depth & nodes & time & depth & nodes \\
\midrule
% lake-8 & 256 & ${<}1$ & 6 & 32 & ${<}1$ & 8 & 40 \\
lake-12 & 576 & 6.7 & 7 & 75 & ${<}1$ & 12 & 73 \\
traffic & 722 & 12.6 & 6 & 28 & ${<}1$ & 12 & 32 \\
% sys-tree & 1024 & 3.0 & 7 & 24 & ${<}1$ & 7 & 12 \\
blackjack & 1066 & ${<}1$ & 4 & 10 & ${<}1$ & 7 & 8 \\
% maze-5 & 1624 & TO & 8 & - & ${<}1$ & 13 & 111 \\
% sys-1 & 2304 & 67.3 & 8 & 101 & ${<}1$ & 8 & 76 \\
sys-2 & 2304 & 62.9 & 8 & 94 & ${<}1$ & 8 & 41 \\
pacman & 2951 & 5.0 & 5 & 22 & ${<}1$ & 14 & 183 \\
% maze-6 & 4012 & TO & 7 & - & ${<}1$ & 14 & 172 \\
\cmidrule(lr){1-8}
wlan & 4189 & TO & 6 & - & ${<}1$ & 11 & 159 \\
ij & 5120 & TO & 8 & - & ${<}1$ & 10 & 645 \\
firewire & 5515 & 20.1 & 5 & 24 & ${<}1$ & 9 & 69 \\
pnueli & 6457 & 7.8 & 6 & 61 & ${<}1$ & 15 & 857 \\
csma & 7988 & TO & 6 & - & ${<}1$ & 9 & 54 \\
maze-7 & 8156 & TO & 7 & - & ${<}1$ & 14 & 280 \\
consensus & 9232 & 12.0 & 5 & 23 & ${<}1$ & 9 & 51 \\
resource & 10571 & ${<}1$ & 3 & 7 & ${<}1$ & 16 & 248 \\
philosophers & 10932 & 13.3 & 6 & 40 & ${<}1$ & 16 & 946 \\
rabin & 15388 & TO & 6 & - & ${<}1$ & 21 & 154 \\
tictactoe & 21816 & TO & 6 & - & 1.4 & 14 & 1170 \\
\bottomrule
\end{tabular}

==> tables/big-omdt-table.tex <==
\begin{tabular}{l cccc@{\hskip 12pt}cccc@{\hskip 12pt}cccc}
\toprule
\multirow{2}{*}{model} &
\multicolumn{4}{c@{\hskip 12pt}}{model info} &
\multicolumn{4}{c@{\hskip 12pt}}{\dtpaynt} &
\multicolumn{4}{c}{\omdt}\\
\cmidrule(lr{1.75em}){2-5}\cmidrule(lr{1.75em}){6-9}\cmidrule(lr){10-13}
& $d$ & $|S|$ & $|Act|$ & $V(\opt{M})$ & value & time & depth & nodes & value & time & depth & nodes \\
\midrule
blackjack & 1 & 533 & 2 & -2.17 & -2.35 & 0.5 & 1 & 1 & -2.35 & 8.0 & 1 & 1 \\
blackjack & 2 & 533 & 2 & -2.17 & -2.21 & 14.2 & 2 & 3 & -2.21 & 12.0 & 2 & 3 \\
blackjack & 3 & 533 & 2 & -2.17 & -2.21 & 14.2 & 2 & 3 & -2.17 & 143.0 & 3 & 7 \\
blackjack & 4 & 533 & 2 & -2.17 & -2.17 & 194.3 & 4 & 11 & -2.17 & 166.0 & 4 & 13 \\
blackjack & 5 & 533 & 2 & -2.17 & -2.17 & 165.4 & 4 & 11 & -2.17 & 432.0 & 5 & 12 \\
blackjack & 6 & 533 & 2 & -2.17 & -2.17 & 144.9 & 4 & 11 & -2.17 & 1089.0 & 6 & 21 \\
lake-8 & 1 & 64 & 4 & 0.41 & 0.31 & 0.1 & 1 & 1 & 0.31 & 0.0 & 1 & 1 \\
lake-8 & 2 & 64 & 4 & 0.41 & 0.39 & 3.6 & 2 & 3 & 0.39 & 3.0 & 2 & 3 \\
lake-8 & 3 & 64 & 4 & 0.41 & 0.39 & 983.6 & 3 & 7 & 0.39 & 11.0 & 3 & 6 \\
lake-8 & 4 & 64 & 4 & 0.41 & 0.39 & 203.4 & 4 & 10 & 0.40 & 520.0 & 4 & 14 \\
lake-8 & 5 & 64 & 4 & 0.41 & 0.39 & 245.2 & 5 & 13 & 0.41 & 1162.0 & 5 & 28 \\
lake-8 & 6 & 64 & 4 & 0.41 & 0.41 & 322.9 & 6 & 36 & 0.41 & 142.0 & 6 & 37 \\
lake-12 & 1 & 144 & 4 & 0.35 & 0.02 & 0.3 & 1 & 1 & 0.02 & 1.0 & 1 & 1 \\
lake-12 & 2 & 144 & 4 & 0.35 & 0.12 & 167.8 & 2 & 3 & 0.12 & 103.0 & 2 & 3 \\
lake-12 & 3 & 144 & 4 & 0.35 & 0.12 & 192.9 & 3 & 6 & 0.24 & 1160.0 & 3 & 6 \\
lake-12 & 4 & 144 & 4 & 0.35 & 0.12 & 301.1 & 4 & 8 & 0.28 & 788.0 & 4 & 14 \\
lake-12 & 5 & 144 & 4 & 0.35 & 0.17 & 511.9 & 4 & 9 & 0.31 & 1167.0 & 5 & 20 \\
lake-12 & 6 & 144 & 4 & 0.35 & 0.15 & 420.6 & 5 & 14 & 0.31 & 1178.0 & 6 & 32 \\
sys-1 & 1 & 256 & 9 & 223.96 & 203.41 & 0.2 & 0 & 0 & 203.42 & 14.0 & 0 & 0 \\
sys-1 & 2 & 256 & 9 & 223.96 & 209.94 & 182.0 & 2 & 2 & 209.95 & 871.0 & 2 & 3 \\
sys-1 & 3 & 256 & 9 & 223.96 & 210.48 & 232.6 & 3 & 5 & 212.10 & 1199.0 & 3 & 7 \\
sys-1 & 4 & 256 & 9 & 223.96 & 211.35 & 1103.4 & 4 & 9 & 212.90 & 1195.0 & 4 & 7 \\
sys-1 & 5 & 256 & 9 & 223.96 & 211.16 & 408.5 & 5 & 9 & 213.83 & 1198.0 & 5 & 12 \\
sys-1 & 6 & 256 & 9 & 223.96 & 211.56 & 1088.4 & 6 & 13 & 213.91 & 1188.0 & 6 & 41 \\
sys-2 & 1 & 256 & 9 & 241.15 & 146.65 & 2.5 & 1 & 1 & 146.65 & 159.0 & 1 & 1 \\
sys-2 & 2 & 256 & 9 & 241.15 & 182.81 & 860.0 & 2 & 3 & 182.82 & 606.0 & 2 & 3 \\
sys-2 & 3 & 256 & 9 & 241.15 & 176.43 & 919.6 & 3 & 5 & 190.92 & 1030.0 & 3 & 6 \\
sys-2 & 4 & 256 & 9 & 241.15 & 173.56 & 21.6 & 2 & 3 & 187.90 & 1193.0 & 4 & 9 \\
sys-2 & 5 & 256 & 9 & 241.15 & 173.56 & 21.1 & 2 & 3 & 203.26 & 947.0 & 5 & 17 \\
sys-2 & 6 & 256 & 9 & 241.15 & 173.56 & 21.2 & 2 & 3 & 196.47 & 1175.0 & 6 & 28 \\
sys-tree & 1 & 128 & 8 & 557.71 & 325.56 & 0.1 & 1 & 1 & 377.93 & 18.0 & 1 & 1 \\
sys-tree & 2 & 128 & 8 & 557.71 & 414.64 & 278.3 & 2 & 3 & 433.82 & 1199.0 & 2 & 3 \\
sys-tree & 3 & 128 & 8 & 557.71 & 485.42 & 1120.0 & 3 & 7 & 467.74 & 468.0 & 3 & 7 \\
sys-tree & 4 & 128 & 8 & 557.71 & 537.42 & 446.6 & 4 & 13 & 536.41 & 1148.0 & 4 & 12 \\
sys-tree & 5 & 128 & 8 & 557.71 & 549.21 & 979.9 & 5 & 18 & 516.81 & 1142.0 & 5 & 18 \\
sys-tree & 6 & 128 & 8 & 557.71 & 555.22 & 842.2 & 6 & 21 & 548.14 & 1157.0 & 6 & 23 \\
tictactoe & 1 & 2424 & 9 & 0.97 & -0.98 & 0.9 & 1 & 1 & -0.76 & 398.0 & 1 & 1 \\
tictactoe & 2 & 2424 & 9 & 0.97 & 0.25 & 875.8 & 2 & 3 & 0.25 & 1088.0 & 2 & 3 \\
tictactoe & 3 & 2424 & 9 & 0.97 & 0.25 & 319.4 & 3 & 3 & -0.16 & 904.0 & 3 & 6 \\
tictactoe & 4 & 2424 & 9 & 0.97 & 0.25 & 274.6 & 3 & 3 & -0.84 & 293.0 & 2 & 2 \\
tictactoe & 5 & 2424 & 9 & 0.97 & 0.45 & 535.7 & 5 & 8 & -0.81 & 12.0 & 1 & 1 \\
tictactoe & 6 & 2424 & 9 & 0.97 & 0.45 & 694.2 & 6 & 11 & -0.81 & 25.0 & 1 & 1 \\
traffic & 1 & 361 & 2 & 2.12 & -72.07 & 0.1 & 1 & 1 & -72.07 & 10.0 & 1 & 1 \\
traffic & 2 & 361 & 2 & 2.12 & -0.22 & 22.4 & 2 & 3 & -0.22 & 110.0 & 2 & 3 \\
traffic & 3 & 361 & 2 & 2.12 & 1.99 & 164.9 & 3 & 6 & 1.00 & 938.0 & 3 & 7 \\
traffic & 4 & 361 & 2 & 2.12 & 2.11 & 221.7 & 4 & 9 & 2.11 & 1184.0 & 4 & 11 \\
traffic & 5 & 361 & 2 & 2.12 & 0.97 & 680.9 & 5 & 9 & 2.12 & 1193.0 & 5 & 18 \\
traffic & 6 & 361 & 2 & 2.12 & 2.12 & 996.2 & 6 & 35 & 2.12 & 1198.0 & 6 & 32 \\
maze-7 & 1 & 2039 & 4 & 5.18 & 1.89 & 2.0 & 1 & 1 & 1.95 & 104.0 & 1 & 1 \\
maze-7 & 2 & 2039 & 4 & 5.18 & 3.25 & 12.7 & 2 & 3 & 2.60 & 335.0 & 2 & 3 \\
maze-7 & 3 & 2039 & 4 & 5.18 & 3.93 & 587.5 & 3 & 6 & 2.82 & 471.0 & 3 & 6 \\
maze-7 & 4 & 2039 & 4 & 5.18 & 4.08 & 387.4 & 4 & 6 & 2.05 & 927.0 & 4 & 10 \\
maze-7 & 5 & 2039 & 4 & 5.18 & 4.15 & 835.4 & 5 & 8 & 2.24 & 1180.0 & 5 & 18 \\
maze-7 & 6 & 2039 & 4 & 5.18 & 4.20 & 1194.2 & 6 & 11 & 1.46 & 1020.0 & 5 & 22 \\
csma & 1 & 7959 & 17 & 0.39 & 0.39 & 14.6 & 1 & 1 & 0.39 & 120.0 & 0 & 0 \\
csma & 2 & 7959 & 17 & 0.39 & 0.39 & 152.7 & 2 & 3 & 0.39 & 1160.0 & 0 & 0 \\
csma & 3 & 7959 & 17 & 0.39 & 0.39 & 146.5 & 2 & 3 & 0.38 & 318.0 & 0 & 0 \\
csma & 4 & 7959 & 17 & 0.39 & 0.39 & 147.2 & 2 & 3 & 0.39 & 1012.0 & 4 & 9 \\
csma & 5 & 7959 & 17 & 0.39 & 0.39 & 158.7 & 2 & 3 & 0.39 & 83.0 & 5 & 5 \\
csma & 6 & 7959 & 17 & 0.39 & 0.39 & 151.0 & 2 & 3 & 0.39 & 175.0 & 6 & 6 \\
firewire & 1 & 4094 & 14 & -70.04 & -70.53 & 25.9 & 1 & 1 & -70.53 & 977.0 & 1 & 1 \\
firewire & 2 & 4094 & 14 & -70.04 & -70.35 & 740.6 & 2 & 3 & -73.37 & 1183.0 & 2 & 3 \\
firewire & 3 & 4094 & 14 & -70.04 & -70.28 & 1178.7 & 3 & 6 & -73.25 & 1131.0 & 3 & 5 \\
firewire & 4 & 4094 & 14 & -70.04 & -70.14 & 574.0 & 4 & 9 & -70.31 & 958.0 & 4 & 11 \\
firewire & 5 & 4094 & 14 & -70.04 & -70.09 & 1161.3 & 5 & 13 & -76.21 & 1190.0 & 5 & 15 \\
firewire & 6 & 4094 & 14 & -70.04 & -70.06 & 890.4 & 6 & 20 & -75.54 & 1094.0 & 6 & 34 \\
ij & 1 & 1024 & 11 & 0.66 & 0.65 & 0.5 & 1 & 1 & 0.65 & 127.0 & 1 & 1 \\
ij & 2 & 1024 & 11 & 0.66 & 0.65 & 21.8 & 2 & 2 & 0.65 & 1062.0 & 2 & 3 \\
ij & 3 & 1024 & 11 & 0.66 & 0.65 & 21.9 & 2 & 2 & 0.65 & 1197.0 & 3 & 6 \\
ij & 4 & 1024 & 11 & 0.66 & 0.65 & 326.1 & 4 & 7 & 0.65 & 1005.0 & 4 & 9 \\
ij & 5 & 1024 & 11 & 0.66 & 0.65 & 1145.2 & 4 & 9 & 0.65 & 140.0 & 4 & 4 \\
ij & 6 & 1024 & 11 & 0.66 & 0.65 & 330.4 & 5 & 10 & 0.65 & 1155.0 & 4 & 5 \\
pnueli & 1 & 1950 & 63 & 0.96 & 0.84 & 180.8 & 1 & 1 & 0.74 & 1084.0 & 0 & 0 \\
pnueli-zuck-3 & 2 & 1950 & 63 & 0.96 & 0.94 & 343.6 & 2 & 3 & 0.60 & 396.0 & 2 & 2 \\
pnueli-zuck-3 & 3 & 1950 & 63 & 0.96 & 0.96 & 412.0 & 3 & 6 & 0.65 & 401.0 & 3 & 3 \\
pnueli-zuck-3 & 4 & 1950 & 63 & 0.96 & 0.88 & 576.4 & 4 & 6 & 0.66 & 822.0 & 3 & 4 \\
pnueli-zuck-3 & 5 & 1950 & 63 & 0.96 & 0.88 & 486.4 & 4 & 6 & 0.66 & 522.0 & 5 & 6 \\
pnueli-zuck-3 & 6 & 1950 & 63 & 0.96 & 0.88 & 411.8 & 4 & 7 & 0.65 & 83.0 & 0 & 0 \\
rabin & 1 & 10241 & 17 & 0.96 & 0.94 & 21.6 & 1 & 1 & 0.92 & 762.0 & 0 & 0 \\
rabin & 2 & 10241 & 17 & 0.96 & 0.96 & 966.2 & 2 & 2 & 0.92 & 12.0 & 0 & 0 \\
rabin & 3 & 10241 & 17 & 0.96 & 0.95 & 1129.9 & 3 & 6 & 0.92 & 557.0 & 3 & 5 \\
rabin & 4 & 10241 & 17 & 0.96 & 0.94 & 206.5 & 2 & 3 & 0.92 & 406.0 & 3 & 3 \\
rabin & 5 & 10241 & 17 & 0.96 & 0.96 & 623.1 & 5 & 7 & 0.92 & 93.0 & 0 & 0 \\
rabin & 6 & 10241 & 17 & 0.96 & 0.96 & 544.6 & 5 & 7 & 0.92 & 200.0 & 0 & 0 \\
resource & 1 & 3292 & 5 & -47.71 & -95.14 & 0.6 & 1 & 1 & -95.14 & 173.0 & 1 & 1 \\
resource & 2 & 3292 & 5 & -47.71 & -53.91 & 34.1 & 2 & 3 & -99.21 & 1096.0 & 2 & 3 \\
resource & 3 & 3292 & 5 & -47.71 & -47.71 & 95.0 & 3 & 4 & -68.63 & 900.0 & 3 & 4 \\
resource & 4 & 3292 & 5 & -47.71 & -47.71 & 98.6 & 3 & 4 & -99.87 & 563.0 & 4 & 10 \\
resource & 5 & 3292 & 5 & -47.71 & -47.71 & 97.8 & 3 & 4 & -99.16 & 566.0 & 5 & 17 \\
resource & 6 & 3292 & 5 & -47.71 & -47.71 & 95.5 & 3 & 4 & -100.00 & 893.0 & 6 & 14 \\
wlan & 1 & 3127 & 34 & 0.11 & 0.05 & 58.7 & 1 & 1 & 0.04 & 631.0 & 1 & 1 \\
wlan & 2 & 3127 & 34 & 0.11 & 0.06 & 354.2 & 2 & 3 & 0.04 & 670.0 & 2 & 2 \\
wlan & 3 & 3127 & 34 & 0.11 & 0.06 & 253.6 & 2 & 3 & 0.04 & 1109.0 & 3 & 6 \\
wlan & 4 & 3127 & 34 & 0.11 & 0.07 & 572.4 & 4 & 9 & 0.04 & 25.0 & 0 & 0 \\
wlan & 5 & 3127 & 34 & 0.11 & 0.07 & 446.1 & 4 & 9 & 0.04 & 1120.0 & 5 & 23 \\
wlan & 6 & 3127 & 34 & 0.11 & 0.07 & 385.3 & 4 & 9 & 0.03 & 1001.0 & 3 & 3 \\
\bottomrule
\end{tabular}


==> tables/dtcontrol-table-sidebyside.tex <==
% \begin{tabular}{l c@{\hskip 8pt}rrr@{\hskip 8pt}rc@{\hskip 24pt} l c@{\hskip 8pt}rrr@{\hskip 8pt}rc}
% \toprule
% \multirow{2}{*}{model} &
% \multicolumn{1}{c@{\hskip 8pt}}{model info} &
% \multicolumn{3}{c@{\hskip 8pt}}{\dtpaynt} &
% \multicolumn{2}{c@{\hskip 24pt}}{{{\dtcontrol}}} &
% \multirow{2}{*}{model} &
% \multicolumn{1}{c@{\hskip 8pt}}{model info} &
% \multicolumn{3}{c@{\hskip 8pt}}{\dtpaynt} &
% \multicolumn{2}{c}{\dtcontrol}\\
% \cmidrule(lr{1.75em}){2-2}\cmidrule(lr{1.75em}){3-5}\cmidrule(lr{3.25em}){6-7}\cmidrule(lr{1.75em}){9-9}\cmidrule(lr{1.75em}){10-12}\cmidrule(lr){13-14}
% & choices & time & d & n & d & n & & choices & time & d & n & d & n \\
% \midrule
% lake-8 & 256 & ${<}1$ & 6 & 32 & 8 & 40 & lake-12 & 576 & 6.7 & 7 & 75 & 12 & 73 \\
% traffic & 722 & 12.6 & 6 & 28 & 12 & 32 & sys-tree & 1024 & 3.0 & 7 & 24 & 7 & 12 \\
% blackjack & 1066 & ${<}1$ & 4 & 10 & 7 & 8 & sys-2 & 2304 & 62.9 & 8 & 94 & 8 & 41 \\
% pacman & 2951 & 5.0 & 5 & 22 & 14 & 183 & maze-6 & 4012 & TO & 7 & - & 14 & 172 \\
% \cmidrule(lr){1-14}
% wlan & 4189 & TO & 6 & - & 11 & 159 & ij & 5120 & TO & 8 & - & 10 & 645 \\
% firewire & 5515 & 20.1 & 5 & 24 & 9 & 69 & pnueli & 6457 & 7.8 & 6 & 61 & 15 & 857 \\
% csma & 7988 & TO & 6 & - & 9 & 54 & maze-7 & 8156 & TO & 7 & - & 14 & 280 \\
% consensus & 9232 & 12.0 & 5 & 23 & 9 & 51 & resource & 10571 & ${<}1$ & 3 & 7 & 16 & 248 \\
% philosophers & 10932 & 13.3 & 6 & 40 & 16 & 946 & rabin & 15388 & TO & 6 & - & 21 & 154 \\
% tictactoe\_vs\_r & 21816 & TO & 6 & - & 14 & 1170 &  &  &  &  &  &  &  \\
% \bottomrule
% \end{tabular}

%milan version 
% \begin{tabular}{l@{\hskip 8pt}rrr@{\hskip 8pt}rr@{\hskip 16pt} l@{\hskip 8pt}rrr@{\hskip 8pt}rr}
% \toprule
% \multirow{2}{*}{model} &
% \multicolumn{3}{c@{\hskip 8pt}}{{\scalebox{0.7}{\dtpaynt}}} &
% \multicolumn{2}{c@{\hskip 16pt}}{{\scalebox{0.7}{\dtcontrol}}} &
% \multirow{2}{*}{model} &
% \multicolumn{3}{c@{\hskip 8pt}}{\scalebox{0.7}{\dtpaynt}} &
% \multicolumn{2}{c}{\scalebox{0.7}{\dtcontrol}}\\
% \cmidrule(lr{1em}){2-4}\cmidrule(lr{2em}){5-6}\cmidrule(lr{1em}){8-10}\cmidrule(lr){11-12}
% & time & d & n & d & n & & time & d & n & d & n \\
% \midrule
% lake-12 (576) & 7 & 7 & 75 & 12 & 73 &  traffic (722) & 13 & 6 & 28 & 12 & 32 \\
% sys-tree (1k) & 3 & 7 & 24 & 7 & 12 & blackjack (1k) & ${<}1$ & 4 & 10 & 7 & 8 \\
% sys-2 (2.3k) & 63 & 8 & 94 & 8 & 41 & pacman (3k) & 5 & 5 & 22 & 14 &  183\\
% \cmidrule(lr){1-12}
% wlan (4.2k) & TO & 6 & - & 11 & 159 & tictactoe (22k) & TO & 6 & - & 14 & 1170  \\
% firewire (5.5k) & 20 & 5 & 24 & 9 & 69 & pnueli (6.5k) & 8 & 6 & 61 & 15 & 857 \\
% csma (8k) & TO & 6 & - & 9 & 54 & maze-7 (8.2k) & TO & 7 & - & 14 & 280 \\
% consensus (9.2k) & 12 & 5 & 23 & 9 & 51 & resource (11k) & ${<}1$ & 3 & 7 & 16 & 248 \\
% philosophers (11k) & 13 & 6 & 40 & 16 & 946 & rabin (15k) & TO & 6 & - & 21 & 154 \\
% %ij & 5120 & TO & 8 & - & 10 & 645 &  &  &  &  &  &  &  \\
% \bottomrule
% \end{tabular}

% \scalebox{0.95}{
% \begin{tabular}{l@{\hskip 6pt}rrr@{\hskip 5pt}crr|@{\hskip 5pt} l@{\hskip 6pt}rrr@{\hskip 5pt}crr}
% \toprule
% \multirow{2}{*}{model} &
% \multicolumn{3}{c@{\hskip 8pt}}{{\scalebox{0.8}{\dtpaynt}}} &
% \multicolumn{3}{c@{\hskip 8pt}}{{\scalebox{0.8}{\dtcontrol}}} &
% \multirow{2}{*}{model} &
% \multicolumn{3}{c@{\hskip 8pt}}{\scalebox{0.8}{\dtpaynt}} &
% \multicolumn{3}{c}{\scalebox{0.8}{\dtcontrol}}\\
% \cmidrule(lr{1em}){2-4}\cmidrule(lr{1em}){5-7}\cmidrule(lr{1em}){9-11}\cmidrule(lr){12-14}
% & time & d & n & & d & n & & time & d & n & & d & n \\
% \midrule
% lake-12 (576) & 7 & 7 & 75 & & 12 & \textbf{73} &  traffic (722) & 13 & 6 & \textbf{28} & & 12 & 32 \\
% sys-tree (1k) & 3 & 7 & 24 & & 7 & \textbf{12} & blackjack (1k) & ${<}1$ & 4 & 10 & & 7 & \textbf{8} \\
% sys-2 (2.3k) & 63 & 8 & 94 & & 8 & \textbf{41} & pacman (3k) & 5 & 5 & \textbf{22} & & 14 &  183\\
% \cmidrule(lr){1-14}
% wlan (4.2k) & TO & ${>}5$ & - & & 11 & \textbf{159} & tictactoe (22k) & TO & ${>}5$ & - & & 14 & \textbf{1170}  \\
% firewire (5.5k) & 20 & 5 & \textbf{24} & & 9 & 69 & pnueli (6.5k) & 8 & 6 & \textbf{61} & & 15 & 857 \\
% csma (8k) & TO & ${>}5$ & - & & 9 & \textbf{54} & maze-7 (8.2k) & TO & ${>}6$ & - & & 14 & \textbf{280} \\
% consensus (9.2k) & 12 & 5 & \textbf{23} & & 9 & 51 & resource (11k) & ${<}1$ & 3 & \textbf{7} & & 16 & 248 \\
% philos (11k) & 13 & 6 & \textbf{40} & & 16 & 946 & rabin (15k) & TO & ${>}5$ & - & & 21 & \textbf{154} \\
% %ij & 5120 & TO & 8 & - & 10 & 645 &  &  &  &  &  &  &  \\
% \bottomrule
% \end{tabular}
% }


\scalebox{0.95}{
\begin{tabular}{l@{\hskip 6pt}rrr@{\hskip 5pt}crr|@{\hskip 5pt} l@{\hskip 6pt}rrr@{\hskip 5pt}crr}
\toprule
\multirow{2}{*}{model} &
\multicolumn{3}{c@{\hskip 8pt}}{{\scalebox{0.85}{\dtmap}}} &
\multicolumn{3}{c@{\hskip 8pt}}{{\scalebox{0.85}{\dtcontrol}}} &
\multirow{2}{*}{model} &
\multicolumn{3}{c@{\hskip 8pt}}{\scalebox{0.85}{\dtmap}} &
\multicolumn{3}{c}{\scalebox{0.85}{\dtcontrol}}\\
\cmidrule(lr{1em}){2-4}\cmidrule(lr{1em}){5-7}\cmidrule(lr{1em}){9-11}\cmidrule(lr){12-14}
& time & $k$ & $n$ & & $k$ & $n$ & & time & $k$ & $n$ & & $k$ & $n$ \\
\midrule
lake-12 (576) & 4 & 7 & \textbf{70} & & 12 & 73 &  traffic (722) & 10.6 & 6 & 34 & & 12 & \textbf{32} \\
%sys-tree (1k) & 3 & 7 & 24 & & 7 & \textbf{12} & blackjack (1k) & ${<}1$ & 4 & 10 & & 7 & \textbf{8} \\
sys-2 (2.3k) & 43 & 8 & 67 & & 8 & \textbf{41} & pacman (3k) & 6 & 5 & \textbf{23} & & 14 &  183\\
\cmidrule(lr){1-14}

firewire (5.5k) & 19 & 5 & \textbf{23} & & 9 & 69 & pnueli (6.5k) & 4 & 6 & \textbf{59} & & 15 & 857 \\
tictactoe (22k) & TO & ${>}5$ & - & & 14 & \textbf{1170}  & maze-7 (8.2k) & TO & ${>}6$ & - & & 14 & \textbf{280} \\
consensus (9.2k) & 14 & 5 & \textbf{22} & & 9 & 51 & resource (11k) & ${<}1$ & 3 & \textbf{7} & & 16 & 248 \\
philos (11k) & 12 & 6 & \textbf{41} & & 16 & 946 & rabin (15k) & TO & ${>}5$ & - & & 21 & \textbf{154} \\
%ij & 5120 & TO & 8 & - & 10 & 645 &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
